Imagine while Reasoning in Space: Multimodal Visualization-of-Thought

Chain-of-Thought (CoT) prompting has proven highly effective for enhancing complex reasoning in Large Language Models (LLMs) and Multimodal Large Language Models (MLLMs). Yet, it struggles in complex spatial reasoning tasks. Nonetheless, human cognition extends beyond language alone, enabling the remarkable capability to think in both words and images. Inspired by this mechanism, we propose a new reasoning paradigm, Multimodal Visualization-of-Thought (MVoT). It enables visual thinking in MLLMs by generating image visualizations of their reasoning traces. To ensure high-quality visualization, we introduce token discrepancy loss into autoregressive MLLMs. This innovation significantly improves both visual coherence and fidelity. We validate this approach through several dynamic spatial reasoning tasks. Experimental results reveal that MVoT demonstrates competitive performance across tasks. Moreover, it exhibits robust and reliable improvements in the most challenging scenarios where CoT fails. Ultimately, MVoT establishes new possibilities for complex reasoning tasks where visual thinking can effectively complement verbal reasoning.

==> CoMT/figs/3_intro_illustraion_fig.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{CoMT/figs/files/intro_1.pdf}
    \caption{Multimodal VoT (MVoT) reasoning strategy visualizes the reasoning process of MLLMs by generating imagined reasoning states in images, leveraging generative models for enhanced spatial reasoning.}
    \label{fig:illustration-mvot}
\end{figure}

==> CoMT/figs/figure-1-maze.tex <==
\begin{figure*}[!hbpt]
    \centering
    \includegraphics[trim={1cm 23cm 2cm 0cm},clip,width=\textwidth]{CoMT/figs/files/figure-1-maze.png}
    \caption{Chain-of-Multimodal-Thought (CoMT) reasoning strategy generates interleaved reasoning traces cross different modalities.}
    \label{fig:illustration-mvot}
\end{figure*}

==> CoMT/tables/3_without_perceptual_loss.tex <==

\begin{table}
\centering
\caption{Task performance of CoMT with and without $\mathcal{L}_p$.}
\renewcommand{\arraystretch}{1.3}
\resizebox{0.55\linewidth}{!}{%
\begin{tabular}{l|ccc} 
\hline
                & \maze   & \minibehavior & \frozenlake  \\ 
\hline
CoMT with $\mathcal{L}_p$   & \textbf{0.9295} & \textbf{0.9514} & \textbf{0.8560}      \\
CoMT without $\mathcal{L}_p$ & 0.7468 & 0.7228 & 0.7206      \\
\hline
\end{tabular}
}
\label{tab:ablation-perceptual-loss}
\end{table}

==> CoMT/tables/prompts/2_mvot_sv.tex <==
\begin{table*}[]
\centering
\caption{Example of input and output for MVoT State Visualization. \textit{Italic} text is the expected response. }
\begin{tcolorbox}[title = {\textbf{MVoT State Visualization}}]
\textbf{\maze}
\\
Task: Maze Navigation Simulation \\
Determine the final destination (A, B, C or D) from the starting point (red point) following the action sequence. The definitions of the actions are as below.  \\
* Go up/left/down/right: move one grid space in the absolute up/left/down/right direction.  \\
Full Action Sequence: Go down. Go left. Go left. Go up. Go up.  \\
Initial maze: \textless image\textgreater \\
Response: Go down. Go left. Go left. \textit{\textless image\textgreater}
% \tcblower
\\
\\
\textbf{\minibehavior}
\\
Task: Mini-Behavior Installing the Printer \\
Determine whether the agent (red triangle) can pick up the printer (printer symbol) on the floor and place it on the table (brown area) and toggle it on. If not, identify the failure reason. The definitions of the actions are as below.  \\
* Go up/left/down/right: move one grid space in the absolute up/left/down/right direction.  \\
* Pick up: pick up the printer from the any of the grid next to the agent. If there is no printer next to the agent, the action fails.  \\
* Drop: drop the printer to the table that is next to the agent. If there is no table next to the agent, the action fails.  \\
* Toggle: toggle the printer that is on the table and next to the agent.  \\
Return A, B, C or D.  \\
Full Action Sequence: Go up. Go up. Go right. Go down. Go down. Pick up. Go right. Drop. Toggle.  \\
A. Action Success.  \\
B. Action Failed: Drop Error.  \\
C. Action Failed: Pick Up Error.  \\
D. Missing Key Objects.  \\
Initial State: \textless image\textgreater Carrying objects: None.   \\
Response: Go up. Go up. Go right. \textit{\textless image\textgreater Carrying objects: None. }
% \tcblower
\\
\\
\textbf{\frozenlake}
\\
Task: FrozenLake \\
Determine whether the agent (elf character) can safely reach the gift following the action sequence without falling into the holes. If not, identify the failure reason. The definitions of the actions are as below. \\
* Go up/left/down/right: move one grid space in the absolute up/left/down/right direction. \\
Return A, B or C. \\
Full Action Sequence: Go right. Go up. \\
A. Action Success. \\
B. Action Failed: Fall into the Hole. \\
C. Action Failed: Agent Safe but Fail to Reach Destination. \\
Initial State: \textless image\textgreater \\
Response: Go right. Go up. \textit{\textless image\textgreater}
\end{tcolorbox}
\label{apptab:mvot-sv-prompt}
\end{table*}

==> CoMT/tables/prompts/3_mvot_ar.tex <==
\begin{table*}[]
\centering
\caption{Example of input and output for MVoT Action Reasoning. \textit{Italic} text is the expected response. }
\begin{tcolorbox}[title = {\textbf{MVoT Action Reasoning}}]
\textbf{\maze}
\\
Task: Maze Navigation Simulation \\
Determine the final destination (A, B, C or D) from the starting point (red point) following the action sequence. The definitions of the actions are as below.  \\
* Go up/left/down/right: move one grid space in the absolute up/left/down/right direction.  \\
Full Action Sequence: Go down. Go left. Go left. Go up. Go up.  \\
Initial maze: \textless image\textgreater \\
Response: Go down. Go left. \textless image\textgreater \textit{Go left. }
\\
\\
\textbf{\minibehavior}
\\
Task: Mini-Behavior Installing the Printer \\
Determine whether the agent (red triangle) can pick up the printer (printer symbol) on the floor and place it on the table (brown area) and toggle it on. If not, identify the failure reason. The definitions of the actions are as below.  \\
* Go up/left/down/right: move one grid space in the absolute up/left/down/right direction.  \\
* Pick up: pick up the printer from the any of the grid next to the agent. If there is no printer next to the agent, the action fails.  \\
* Drop: drop the printer to the table that is next to the agent. If there is no table next to the agent, the action fails.  \\
* Toggle: toggle the printer that is on the table and next to the agent.  \\
Return A, B, C or D.  \\
Full Action Sequence: Go up. Go up. Go right. Go down. Go down. Pick up. Go right. Drop. Toggle.  \\
A. Action Success.  \\
B. Action Failed: Drop Error.  \\
C. Action Failed: Pick Up Error.  \\
D. Missing Key Objects.  \\
Initial State: \textless image\textgreater Carrying objects: None.  \\
Response: Go up. Go up. \textless image\textgreater Carrying objects: None. \textit{Go right. }
% \tcblower
\\
\\
\textbf{\frozenlake}
\\
Task: FrozenLake \\
Determine whether the agent (elf character) can safely reach the gift following the action sequence without falling into the holes. If not, identify the failure reason. The definitions of the actions are as below. \\
* Go up/left/down/right: move one grid space in the absolute up/left/down/right direction. \\
Return A, B or C. \\
Full Action Sequence: Go right. Go up. \\
A. Action Success. \\
B. Action Failed: Fall into the Hole. \\
C. Action Failed: Agent Safe but Fail to Reach Destination. \\
Initial State: \textless image\textgreater \\
Response: Go right. Go up. \textless image\textgreater \textit{The answer is A. }
\end{tcolorbox}
\label{apptab:mvot-ar-prompt}
\end{table*}
